Heavy Higgs Boson Production at Colliders in the Singlet-Triplet Scotogenic Dark Matter Model

We consider the possibility that the dark matter particle is a scalar WIMP messenger associated to neutrino mass generation, made stable by the same symmetry responsible for the radiative origin of neutrino mass. We focus on some of the implications of this proposal as realized within the singlet-triplet scotogenic dark matter model.We identify consistent parameter sets consistent both with neutrino mass and the observed dark matter abundance. Finally we characterize the expected phenomenological profile of heavy Higgs boson physics at the LHC as well as at future linear Colliders.

==> VerticesFFS.tex <==
\begin{center} 
\begin{fmffile}{Diagrams/FeynDia101} 
\fmfframe(20,20)(20,20){ 
\begin{fmfgraph*}(75,75) 
\fmfleft{l1}
\fmfright{r1,r2}
\fmf{fermion}{v1,l1}
\fmf{fermion}{r1,v1}
\fmf{dashes}{r2,v1}
\fmflabel{$\bar{d}_{{i \alpha}}$}{l1}
\fmflabel{$d_{{j \beta}}$}{r1}
\fmflabel{$A^0$}{r2}
\end{fmfgraph*}} 
\end{fmffile} 
\end{center}  
\begin{align} 
 &\frac{1}{\sqrt{2}} \delta_{\alpha \beta} \sum_{b=1}^{3}U^{d,*}_{L,{j b}} \sum_{a=1}^{3}U^{d,*}_{R,{i a}} Y_{d,{a b}}   \Big(\frac{1-\gamma_5}{2}\Big)\\ 
  & + \,- \frac{1}{\sqrt{2}} \delta_{\alpha \beta} \sum_{b=1}^{3}\sum_{a=1}^{3}Y^*_{d,{a b}} U_{R,{j a}}^{d}  U_{L,{i b}}^{d}  \Big(\frac{1+\gamma_5}{2}\Big)\end{align} 
\hrule 
\begin{center} 
\begin{fmffile}{Diagrams/FeynDia102} 
\fmfframe(20,20)(20,20){ 
\begin{fmfgraph*}(75,75) 
\fmfleft{l1}
\fmfright{r1,r2}
\fmf{fermion}{v1,l1}
\fmf{fermion}{r1,v1}
\fmf{dashes}{r2,v1}
\fmflabel{$\bar{e}_{{i}}$}{l1}
\fmflabel{$e_{{j}}$}{r1}
\fmflabel{$A^0$}{r2}
\end{fmfgraph*}} 
\end{fmffile} 
\end{center}  
\begin{align} 
 &\frac{1}{\sqrt{2}} \sum_{b=1}^{3}U^{e,*}_{L,{j b}} \sum_{a=1}^{3}U^{e,*}_{R,{i a}} Y_{e,{a b}}   \Big(\frac{1-\gamma_5}{2}\Big)\\ 
  & + \,- \frac{1}{\sqrt{2}} \sum_{b=1}^{3}\sum_{a=1}^{3}Y^*_{e,{a b}} U_{R,{j a}}^{e}  U_{L,{i b}}^{e}  \Big(\frac{1+\gamma_5}{2}\Big)\end{align} 
\hrule 
\begin{center} 
\begin{fmffile}{Diagrams/FeynDia103} 
\fmfframe(20,20)(20,20){ 
\begin{fmfgraph*}(75,75) 
\fmfleft{l1}
\fmfright{r1,r2}
\fmf{fermion}{v1,l1}
\fmf{fermion}{r1,v1}
\fmf{dashes}{r2,v1}
\fmflabel{$\bar{u}_{{i \alpha}}$}{l1}
\fmflabel{$u_{{j \beta}}$}{r1}
\fmflabel{$A^0$}{r2}
\end{fmfgraph*}} 
\end{fmffile} 
\end{center}  
\begin{align} 
 &\frac{1}{\sqrt{2}} \delta_{\alpha \beta} \sum_{b=1}^{3}U^{u,*}_{L,{j b}} \sum_{a=1}^{3}U^{u,*}_{R,{i a}} Y_{u,{a b}}   \Big(\frac{1-\gamma_5}{2}\Big)\\ 
  & + \,- \frac{1}{\sqrt{2}} \delta_{\alpha \beta} \sum_{b=1}^{3}\sum_{a=1}^{3}Y^*_{u,{a b}} U_{R,{j a}}^{u}  U_{L,{i b}}^{u}  \Big(\frac{1+\gamma_5}{2}\Big)\end{align} 
\hrule 
\begin{center} 
\begin{fmffile}{Diagrams/FeynDia104} 
\fmfframe(20,20)(20,20){ 
\begin{fmfgraph*}(75,75) 
\fmfleft{l1}
\fmfright{r1,r2}
\fmf{plain}{l1,v1}
\fmf{fermion}{r1,v1}
\fmf{scalar}{v1,r2}
\fmflabel{$\chi^0_{{i}}$}{l1}
\fmflabel{$\chi^-$}{r1}
\fmflabel{$H^+_{{k}}$}{r2}
\end{fmfgraph*}} 
\end{fmffile} 
\end{center}  
\begin{align} 
 &2 i Y_\Omega Z^{{\chi^0},*}_{i 2} Z_{{k 2}}^{P} \Big(\frac{1-\gamma_5}{2}\Big)\\ 
  & + \,2 i Y_\Omega^* Z_{{k 2}}^{P} Z_{{i 2}}^{\chi^0} \Big(\frac{1+\gamma_5}{2}\Big)\end{align} 
\hrule 
\begin{center} 
\begin{fmffile}{Diagrams/FeynDia105} 
\fmfframe(20,20)(20,20){ 
\begin{fmfgraph*}(75,75) 
\fmfleft{l1}
\fmfright{r1,r2}
\fmf{plain}{l1,v1}
\fmf{plain}{r1,v1}
\fmf{dashes}{r2,v1}
\fmflabel{$\chi^0_{{i}}$}{l1}
\fmflabel{$\chi^0_{{j}}$}{r1}
\fmflabel{$h_{{k}}$}{r2}
\end{fmfgraph*}} 
\end{fmffile} 
\end{center}  
\begin{align} 
 &2 i Y_\Omega Z^{{H},*}_{k 2} \Big(Z^{{\chi^0},*}_{i 1} Z^{{\chi^0},*}_{j 2}  + Z^{{\chi^0},*}_{i 2} Z^{{\chi^0},*}_{j 1} \Big)\Big(\frac{1-\gamma_5}{2}\Big)\\ 
  & + \,2 i Y_\Omega^* Z^{{H},*}_{k 2} \Big(Z_{{i 1}}^{\chi^0} Z_{{j 2}}^{\chi^0}  + Z_{{i 2}}^{\chi^0} Z_{{j 1}}^{\chi^0} \Big)\Big(\frac{1+\gamma_5}{2}\Big)\end{align} 
\hrule 
\begin{center} 
\begin{fmffile}{Diagrams/FeynDia106} 
\fmfframe(20,20)(20,20){ 
\begin{fmfgraph*}(75,75) 
\fmfleft{l1}
\fmfright{r1,r2}
\fmf{plain}{l1,v1}
\fmf{plain}{r1,v1}
\fmf{dashes}{r2,v1}
\fmflabel{$\chi^0_{{i}}$}{l1}
\fmflabel{$\nu_{{j}}$}{r1}
\fmflabel{$\eta_i$}{r2}
\end{fmfgraph*}} 
\end{fmffile} 
\end{center}  
\begin{align} 
 &\frac{1}{\sqrt{2}} Z^{{\chi^0},*}_{i 2} \sum_{a=1}^{3}U^{V,*}_{j a} Y_{N,{a}}  \Big(\frac{1-\gamma_5}{2}\Big)\\ 
  & + \,- \frac{1}{\sqrt{2}} \sum_{a=1}^{3}Y^*_{N,{a}} U_{{j a}}^{V}  Z_{{i 2}}^{\chi^0} \Big(\frac{1+\gamma_5}{2}\Big)\end{align} 
\hrule 
\begin{center} 
\begin{fmffile}{Diagrams/FeynDia107} 
\fmfframe(20,20)(20,20){ 
\begin{fmfgraph*}(75,75) 
\fmfleft{l1}
\fmfright{r1,r2}
\fmf{plain}{l1,v1}
\fmf{fermion}{r1,v1}
\fmf{scalar}{r2,v1}
\fmflabel{$\chi^0_{{i}}$}{l1}
\fmflabel{$e_{{j}}$}{r1}
\fmflabel{$\eta^+$}{r2}
\end{fmfgraph*}} 
\end{fmffile} 
\end{center}  
\begin{align} 
 &i Z^{{\chi^0},*}_{i 2} \sum_{a=1}^{3}U^{e,*}_{L,{j a}} Y_{N,{a}}  \Big(\frac{1-\gamma_5}{2}\Big)\end{align} 
\hrule 
\begin{center} 
\begin{fmffile}{Diagrams/FeynDia108} 
\fmfframe(20,20)(20,20){ 
\begin{fmfgraph*}(75,75) 
\fmfleft{l1}
\fmfright{r1,r2}
\fmf{plain}{l1,v1}
\fmf{plain}{r1,v1}
\fmf{dashes}{r2,v1}
\fmflabel{$\chi^0_{{i}}$}{l1}
\fmflabel{$\nu_{{j}}$}{r1}
\fmflabel{$\eta_R$}{r2}
\end{fmfgraph*}} 
\end{fmffile} 
\end{center}  
\begin{align} 
 &-i \frac{1}{\sqrt{2}} Z^{{\chi^0},*}_{i 2} \sum_{a=1}^{3}U^{V,*}_{j a} Y_{N,{a}}  \Big(\frac{1-\gamma_5}{2}\Big)\\ 
  & + \,-i \frac{1}{\sqrt{2}} \sum_{a=1}^{3}Y^*_{N,{a}} U_{{j a}}^{V}  Z_{{i 2}}^{\chi^0} \Big(\frac{1+\gamma_5}{2}\Big)\end{align} 
\hrule 
\begin{center} 
\begin{fmffile}{Diagrams/FeynDia109} 
\fmfframe(20,20)(20,20){ 
\begin{fmfgraph*}(75,75) 
\fmfleft{l1}
\fmfright{r1,r2}
\fmf{fermion}{v1,l1}
\fmf{plain}{r1,v1}
\fmf{scalar}{r2,v1}
\fmflabel{$\bar{\chi}^-$}{l1}
\fmflabel{$\chi^0_{{j}}$}{r1}
\fmflabel{$H^-_{{k}}$}{r2}
\end{fmfgraph*}} 
\end{fmffile} 
\end{center}  
\begin{align} 
 &2 i Y_\Omega Z^{{P},*}_{k 2} Z^{{\chi^0},*}_{j 2} \Big(\frac{1-\gamma_5}{2}\Big)\\ 
  & + \,2 i Y_\Omega^* Z^{{P},*}_{k 2} Z_{{j 2}}^{\chi^0} \Big(\frac{1+\gamma_5}{2}\Big)\end{align} 
\hrule 
\begin{center} 
\begin{fmffile}{Diagrams/FeynDia110} 
\fmfframe(20,20)(20,20){ 
\begin{fmfgraph*}(75,75) 
\fmfleft{l1}
\fmfright{r1,r2}
\fmf{fermion}{v1,l1}
\fmf{plain}{r1,v1}
\fmf{scalar}{v1,r2}
\fmflabel{$\bar{e}_{{i}}$}{l1}
\fmflabel{$\chi^0_{{j}}$}{r1}
\fmflabel{$\eta^{+,*}$}{r2}
\end{fmfgraph*}} 
\end{fmffile} 
\end{center}  
\begin{align} 
 &\\ 
  & + \,i \sum_{a=1}^{3}Y^*_{N,{a}} U_{L,{i a}}^{e}  Z_{{j 2}}^{\chi^0} \Big(\frac{1+\gamma_5}{2}\Big)\end{align} 
\hrule 
\begin{center} 
\begin{fmffile}{Diagrams/FeynDia111} 
\fmfframe(20,20)(20,20){ 
\begin{fmfgraph*}(75,75) 
\fmfleft{l1}
\fmfright{r1,r2}
\fmf{fermion}{v1,l1}
\fmf{fermion}{r1,v1}
\fmf{dashes}{r2,v1}
\fmflabel{$\bar{d}_{{i \alpha}}$}{l1}
\fmflabel{$d_{{j \beta}}$}{r1}
\fmflabel{$h_{{k}}$}{r2}
\end{fmfgraph*}} 
\end{fmffile} 
\end{center}  
\begin{align} 
 &i \frac{1}{\sqrt{2}} Z^{{H},*}_{k 1} \delta_{\alpha \beta} \sum_{b=1}^{3}U^{d,*}_{L,{j b}} \sum_{a=1}^{3}U^{d,*}_{R,{i a}} Y_{d,{a b}}   \Big(\frac{1-\gamma_5}{2}\Big)\\ 
  & + \,i \frac{1}{\sqrt{2}} Z^{{H},*}_{k 1} \delta_{\alpha \beta} \sum_{b=1}^{3}\sum_{a=1}^{3}Y^*_{d,{a b}} U_{R,{j a}}^{d}  U_{L,{i b}}^{d}  \Big(\frac{1+\gamma_5}{2}\Big)\end{align} 
\hrule 
\begin{center} 
\begin{fmffile}{Diagrams/FeynDia112} 
\fmfframe(20,20)(20,20){ 
\begin{fmfgraph*}(75,75) 
\fmfleft{l1}
\fmfright{r1,r2}
\fmf{fermion}{v1,l1}
\fmf{fermion}{r1,v1}
\fmf{scalar}{v1,r2}
\fmflabel{$\bar{u}_{{i \alpha}}$}{l1}
\fmflabel{$d_{{j \beta}}$}{r1}
\fmflabel{$H^+_{{k}}$}{r2}
\end{fmfgraph*}} 
\end{fmffile} 
\end{center}  
\begin{align} 
 &i \delta_{\alpha \beta} \sum_{b=1}^{3}U^{d,*}_{L,{j b}} \sum_{a=1}^{3}U^{u,*}_{R,{i a}} Y_{u,{a b}}   Z_{{k 1}}^{P} \Big(\frac{1-\gamma_5}{2}\Big)\\ 
  & + \,i \delta_{\alpha \beta} \sum_{b=1}^{3}\sum_{a=1}^{3}Y^*_{d,{a b}} U_{R,{j a}}^{d}  U_{L,{i b}}^{u}  Z_{{k 1}}^{P} \Big(\frac{1+\gamma_5}{2}\Big)\end{align} 
\hrule 
\begin{center} 
\begin{fmffile}{Diagrams/FeynDia113} 
\fmfframe(20,20)(20,20){ 
\begin{fmfgraph*}(75,75) 
\fmfleft{l1}
\fmfright{r1,r2}
\fmf{plain}{l1,v1}
\fmf{fermion}{r1,v1}
\fmf{scalar}{v1,r2}
\fmflabel{$\nu_{{i}}$}{l1}
\fmflabel{$e_{{j}}$}{r1}
\fmflabel{$H^+_{{k}}$}{r2}
\end{fmfgraph*}} 
\end{fmffile} 
\end{center}  
\begin{align} 
 &\\ 
  & + \,i \sum_{b=1}^{3}\sum_{a=1}^{3}Y^*_{e,{a b}} U_{R,{j a}}^{e}  U_{{i b}}^{V}  Z_{{k 1}}^{P} \Big(\frac{1+\gamma_5}{2}\Big)\end{align} 
\hrule 
\begin{center} 
\begin{fmffile}{Diagrams/FeynDia114} 
\fmfframe(20,20)(20,20){ 
\begin{fmfgraph*}(75,75) 
\fmfleft{l1}
\fmfright{r1,r2}
\fmf{fermion}{v1,l1}
\fmf{fermion}{r1,v1}
\fmf{dashes}{r2,v1}
\fmflabel{$\bar{e}_{{i}}$}{l1}
\fmflabel{$e_{{j}}$}{r1}
\fmflabel{$h_{{k}}$}{r2}
\end{fmfgraph*}} 
\end{fmffile} 
\end{center}  
\begin{align} 
 &i \frac{1}{\sqrt{2}} Z^{{H},*}_{k 1} \sum_{b=1}^{3}U^{e,*}_{L,{j b}} \sum_{a=1}^{3}U^{e,*}_{R,{i a}} Y_{e,{a b}}   \Big(\frac{1-\gamma_5}{2}\Big)\\ 
  & + \,i \frac{1}{\sqrt{2}} Z^{{H},*}_{k 1} \sum_{b=1}^{3}\sum_{a=1}^{3}Y^*_{e,{a b}} U_{R,{j a}}^{e}  U_{L,{i b}}^{e}  \Big(\frac{1+\gamma_5}{2}\Big)\end{align} 
\hrule 
\begin{center} 
\begin{fmffile}{Diagrams/FeynDia115} 
\fmfframe(20,20)(20,20){ 
\begin{fmfgraph*}(75,75) 
\fmfleft{l1}
\fmfright{r1,r2}
\fmf{fermion}{v1,l1}
\fmf{fermion}{r1,v1}
\fmf{dashes}{r2,v1}
\fmflabel{$\bar{u}_{{i \alpha}}$}{l1}
\fmflabel{$u_{{j \beta}}$}{r1}
\fmflabel{$h_{{k}}$}{r2}
\end{fmfgraph*}} 
\end{fmffile} 
\end{center}  
\begin{align} 
 &-i \frac{1}{\sqrt{2}} Z^{{H},*}_{k 1} \delta_{\alpha \beta} \sum_{b=1}^{3}U^{u,*}_{L,{j b}} \sum_{a=1}^{3}U^{u,*}_{R,{i a}} Y_{u,{a b}}   \Big(\frac{1-\gamma_5}{2}\Big)\\ 
  & + \,-i \frac{1}{\sqrt{2}} Z^{{H},*}_{k 1} \delta_{\alpha \beta} \sum_{b=1}^{3}\sum_{a=1}^{3}Y^*_{u,{a b}} U_{R,{j a}}^{u}  U_{L,{i b}}^{u}  \Big(\frac{1+\gamma_5}{2}\Big)\end{align} 
\hrule 
\begin{center} 
\begin{fmffile}{Diagrams/FeynDia116} 
\fmfframe(20,20)(20,20){ 
\begin{fmfgraph*}(75,75) 
\fmfleft{l1}
\fmfright{r1,r2}
\fmf{fermion}{v1,l1}
\fmf{fermion}{r1,v1}
\fmf{scalar}{r2,v1}
\fmflabel{$\bar{d}_{{i \alpha}}$}{l1}
\fmflabel{$u_{{j \beta}}$}{r1}
\fmflabel{$H^-_{{k}}$}{r2}
\end{fmfgraph*}} 
\end{fmffile} 
\end{center}  
\begin{align} 
 &i Z^{{P},*}_{k 1} \delta_{\alpha \beta} \sum_{b=1}^{3}U^{u,*}_{L,{j b}} \sum_{a=1}^{3}U^{d,*}_{R,{i a}} Y_{d,{a b}}   \Big(\frac{1-\gamma_5}{2}\Big)\\ 
  & + \,i Z^{{P},*}_{k 1} \delta_{\alpha \beta} \sum_{b=1}^{3}\sum_{a=1}^{3}Y^*_{u,{a b}} U_{R,{j a}}^{u}  U_{L,{i b}}^{d}  \Big(\frac{1+\gamma_5}{2}\Big)\end{align} 
\hrule 
\begin{center} 
\begin{fmffile}{Diagrams/FeynDia117} 
\fmfframe(20,20)(20,20){ 
\begin{fmfgraph*}(75,75) 
\fmfleft{l1}
\fmfright{r1,r2}
\fmf{fermion}{v1,l1}
\fmf{plain}{r1,v1}
\fmf{scalar}{r2,v1}
\fmflabel{$\bar{e}_{{i}}$}{l1}
\fmflabel{$\nu_{{j}}$}{r1}
\fmflabel{$H^-_{{k}}$}{r2}
\end{fmfgraph*}} 
\end{fmffile} 
\end{center}  
\begin{align} 
 &i Z^{{P},*}_{k 1} \sum_{b=1}^{3}U^{V,*}_{j b} \sum_{a=1}^{3}U^{e,*}_{R,{i a}} Y_{e,{a b}}   \Big(\frac{1-\gamma_5}{2}\Big)\end{align} 
\hrule 


==> refs-mad <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{thebibliography}{99}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  
%\cite{Hirsch:2013ola}
\bibitem{Hirsch:2013ola}
  M.~Hirsch, R.~A.~Lineros, S.~Morisi, J.~Palacio, N.~Rojas and J.~W.~F.~Valle,
  %``WIMP dark matter as radiative neutrino mass messenger,''
  JHEP {\bf 1310} (2013) 149
  doi:10.1007/JHEP10(2013)149
  [arXiv:1307.8134 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP10(2013)149;%%
  %18 citations counted in INSPIRE as of 17 Oct 2016  
  
%\cite{Merle:2016scw}
\bibitem{Merle:2016scw}
  A.~Merle, M.~Platscher, N.~Rojas, J.~W.~F.~Valle and A.~Vicente,
  %``Consistency of WIMP Dark Matter as radiative neutrino mass messenger,''
  JHEP {\bf 1607} (2016) 013
  doi:10.1007/JHEP07(2016)013
  [arXiv:1603.05685 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP07(2016)013;%%
  %7 citations counted in INSPIRE as of 22 Oct 2016

  %\cite{Casas:2001sr}
\bibitem{Casas:2001sr} 
  J.~A.~Casas and A.~Ibarra,
  %``Oscillating neutrinos and muon ---> e, gamma,''
  Nucl.\ Phys.\ B {\bf 618}, 171 (2001)
  doi:10.1016/S0550-3213(01)00475-8
  [hep-ph/0103065].
  %%CITATION = doi:10.1016/S0550-3213(01)00475-8;%%
  %739 citations counted in INSPIRE as of 14 Nov 2016

%\cite{Aad:2015zhl}
\bibitem{Aad:2015zhl} 
  G.~Aad {\it et al.} [ATLAS and CMS Collaborations],
  %``Combined Measurement of the Higgs Boson Mass in $pp$ Collisions at $\sqrt{s}=7$ and 8 TeV with the ATLAS and CMS Experiments,''
  Phys.\ Rev.\ Lett.\  {\bf 114}, 191803 (2015)
  doi:10.1103/PhysRevLett.114.191803
  [arXiv:1503.07589 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevLett.114.191803;%%
  %409 citations counted in INSPIRE as of 30 May 2016

%\cite{Bennett:2012zja}
\bibitem{Bennett:2012zja} 
  C.~L.~Bennett {\it et al.} [WMAP Collaboration],
  %``Nine-Year Wilkinson Microwave Anisotropy Probe (WMAP) Observations: Final Maps and Results,''
  Astrophys.\ J.\ Suppl.\  {\bf 208}, 20 (2013)
  doi:10.1088/0067-0049/208/2/20
  [arXiv:1212.5225 [astro-ph.CO]].
  %%CITATION = doi:10.1088/0067-0049/208/2/20;%%
  %1008 citations counted in INSPIRE as of 15 Nov 2016

%\cite{Ade:2015xua}
\bibitem{Ade:2015xua} 
  P.~A.~R.~Ade {\it et al.} [Planck Collaboration],
  %``Planck 2015 results. XIII. Cosmological parameters,''
  Astron.\ Astrophys.\  {\bf 594}, A13 (2016)
  doi:10.1051/0004-6361/201525830
  [arXiv:1502.01589 [astro-ph.CO]].
  %%CITATION = doi:10.1051/0004-6361/201525830;%%
  %2411 citations counted in INSPIRE as of 15 Nov 201

%\cite{Diaz:2015pyv}
\bibitem{Diaz:2015pyv} 
  M.~A.~D\'\i az, B.~Koch and S.~Urrutia-Quiroga,
  %``Constraints to Dark Matter from Inert Higgs Doublet Model,''
  Adv.\ High Energy Phys.\  {\bf 2016}, 8278375 (2016)
  doi:10.1155/2016/8278375
  [arXiv:1511.04429 [hep-ph]].
  %%CITATION = doi:10.1155/2016/8278375;%%
  %8 citations counted in INSPIRE as of 15 Nov 2016
  
%\cite{Forero:2014bxa}
\bibitem{Forero:2014bxa} 
  D.~V.~Forero, M.~Tortola and J.~W.~F.~Valle,
  %``Neutrino oscillations refitted,''
  Phys.\ Rev.\ D {\bf 90}, no. 9, 093006 (2014)
  doi:10.1103/PhysRevD.90.093006
  [arXiv:1405.7540 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.90.093006;%%
  %379 citations counted in INSPIRE as of 15 Nov 2016

%\cite{Alwall:2014hca}
\bibitem{Alwall:2014hca} 
  J.~Alwall {\it et al.},
  %``The automated computation of tree-level and next-to-leading order differential cross sections, and their matching to parton shower simulations,''
  JHEP {\bf 1407}, 079 (2014)
  doi:10.1007/JHEP07(2014)079
  [arXiv:1405.0301 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP07(2014)079;%%
  %1084 citations counted in INSPIRE as of 15 Jul 2016
  
%\cite{Baer:2013cma}
\bibitem{Baer:2013cma} 
  H.~Baer {\it et al.},
  %``The International Linear Collider Technical Design Report - Volume 2: Physics,''
  arXiv:1306.6352 [hep-ph].
  %%CITATION = ARXIV:1306.6352;%%
  %400 citations counted in INSPIRE as of 30 Sep 2016

%\cite{Abramowicz:2013tzc}
\bibitem{Abramowicz:2013tzc} 
  H.~Abramowicz {\it et al.} [CLIC Detector and Physics Study Collaboration],
  %``Physics at the CLIC e+e- Linear Collider -- Input to the Snowmass process 2013,''
  arXiv:1307.5288 [hep-ex].
  %%CITATION = ARXIV:1307.5288;%%
  %61 citations counted in INSPIRE as of 06 Jun 2016
  
%\cite{Blunier:2016peh}
\bibitem{Blunier:2016peh} 
  S.~Blunier, G.~Cottin, M.~A.~D\'\i az and B.~Koch,
  %``Phenomenology of a Higgs triplet model at future $e^{+}e^{-}$ colliders,''
  arXiv:1611.07896 [hep-ph].
  %%CITATION = ARXIV:1611.07896;%%

%\cite{Porod:2003um}
\bibitem{Porod:2003um} 
  W.~Porod,
  %``SPheno, a program for calculating supersymmetric spectra, SUSY particle decays and SUSY particle production at e+ e- colliders,''
  Comput.\ Phys.\ Commun.\  {\bf 153}, 275 (2003)
  doi:10.1016/S0010-4655(03)00222-4
  [hep-ph/0301101].
  %%CITATION = doi:10.1016/S0010-4655(03)00222-4;%%
  %669 citations counted in INSPIRE as of 17 Nov 2016
  
%\cite{Gunion:1989we}
\bibitem{Gunion:1989we}
  J.~F.~Gunion, H.~E.~Haber, G.~L.~Kane and S.~Dawson,
  %``The Higgs Hunter's Guide,''
  Front.\ Phys.\  {\bf 80} (2000) 1.
  %%CITATION = FRPHA,80,1;%%
  %607 citations counted in INSPIRE as of 04 Dec 2016
%\cite{Gunion:1992hs}
%%\bibitem{Gunion:1992hs}
  J.~F.~Gunion, H.~E.~Haber, G.~L.~Kane and S.~Dawson,
  %``Errata for the Higgs hunter's guide,''
  hep-ph/9302272.
  %%CITATION = HEP-PH/9302272;%%
  %151 citations counted in INSPIRE as of 04 Dec 2016
  
\end{thebibliography}


